On the Convergence of Alternating Least Squares Optimisation in Tensor Format Representations

The approximation of tensors is important for the efficient numerical treatment of high dimensional problems, but it remains an extremely challenging task. One of the most popular approach to tensor approximation is the alternating least squares method. In our study, the convergence of the alternating least squares algorithm is considered. The analysis is done for arbitrary tensor format representations and based on the multiliearity of the tensor format. In tensor format representation techniques, tensors are approximated by multilinear combinations of objects lower dimensionality. The resulting reduction of dimensionality not only reduces the amount of required storage but also the computational effort.

==> MATHS/PRE_MATH.TEX <==
%%%%% Begin  LaTeX  File PRE_MATH.tex             5. Feb. 96  %%%%%%%%%%%%%%%%%
%%%%%
%%%%% Definieren mathematischer Zusatzzeichen   und Symbole
%%%%%
%%%%%            based on HEADMATH.tex      Edgar Katzer, Hamburg, Sept. 1995.
%%%%%
%%%%%            and      AMMACROS.tex     (angewandte Mathematik Hamburg) 10. 11. 89
%%%%%                     PRE_VOSS.tex      H. VOSS, Sven Loges (9/89, 10/89) Mathematik TU-Harburg
%%%%%
%%%%% Author:    Edgar Katzer, Hamburg
%%%%% Version:   Version of 11. Dec, 1995,
%%%%%
%
%
%%%%%%%%%%%%%%%%%  Spezielle mathematische Zeichen       %%%%%%
%
%
%%  Mengensymbole
%
    \newcommand    {\BbbC}  {\mbox{\rm $\scriptscriptstyle    %%  complex C
                                   ^\mid$\hspace{-0.40em}C}}
    \newcommand    {\BbbN}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}N}}
    \newcommand    {\BbbK}  {\mbox{                           %%  integer N
                            \rm I\hspace{-0.22em}I\hspace{-0.32em}K}}
    \newcommand    {\BbbQ}  {\mbox{\rm $\scriptscriptstyle    %%  rational Q
                                   ^\mid$\hspace{-0.40em}Q}}
    \newcommand    {\BbbR}  {\mbox{\rm I\hspace{-0.22em}R}}   %%  real    IR
    \newcommand    {\BbbE}  {\mbox{\rm I\hspace{-0.22em}E}}   %%  euclidian IE
    \newcommand    {\BbbZ}  {\mbox{\sf Z\hspace{-0.44em}Z}}   %%  integer Z

    \newcommand    {\icom}  {\BbbC}                           %%  complex C
    \newcommand    {\inat}  {\BbbN}                           %%  integer N
    \newcommand    {\irat}  {\BbbQ}                           %%  rational Q
    \newcommand    {\iree}  {\BbbR}                           %%  real    IR
    \newcommand    {\znat}  {\BbbZ}                           %%  integer Z

    \newcommand    {\nin}   {\in \hspace{-0.80em} /}       %%  not in
%
%   from  AMMACROS.tex   10.11.89
%
 %  \def            \R      {\mbox{\makebox[.2em][l]{I}R}}
 %  \def            \B      {\mbox{\makebox[.2em][l]{I}B}}
 %  \def            \N      {\mbox{\makebox[.2em][l]{I}N}}
 %  \def            \Z      {\mbox{\makebox[.22em][l]{\sf Z}{\sf Z}}}
               %\def\Z{\mbox{\makebox[.283em][l]{Z}Z}}
 %  \def            \C      {\makebox[.6em]{\makebox[-.18em]{C}\rule{.03em}{1.5ex}}}
               %\def\C{\makebox[.8em][l]{\makebox[.25em][l]{C}\rule{.03em}{1.5ex}}}
 %  \def            \Q      {\makebox[.6em]{\makebox[-.25em]{Q}\rule{.03em}{1.5ex}}}
               %\def\Q      {\makebox[.8em][l]{\makebox[.25em][l]{Q}\rule{.03em}{1.5ex}}}
    \def            \L      {\mbox{\makebox[.2em][l]{I}L}}
    \def            \P      {\mbox{\makebox[.2em][l]{I}P}}
%
%%  Spezielle Schriftarten  ( FETT,  \sf   etc
%
    \newcommand    {\ZZ}    { \mbox{\rm\bf{Z}} }
    \newcommand    {\HH}    { {^{\mbox{\scriptsize \sf H }}} }
    \newcommand    {\TT}    { {^{\mbox{\scriptsize \sf T }}} }
%
%
%%%%%%%%%%%%%%%%%  mathematische Begriffe                 %%%%%
%
    \newcommand    {\Bild}  { \mbox{\rm Bild$\,$} }
    \newcommand    {\Kern}  { \mbox{\rm Kernel$\,$} }
    \newcommand    {\Range} { \mbox{\rm Range$\,$} }
    \newcommand    {\Diag}  { \mbox{\rm diag$\,$} }
    \newcommand    {\cond}  { \mbox{\rm cond} }
    \newcommand    {\Span}  { \mbox{\rm Span$\,$} }

    \newcommand    {\Ccone} { \mbox{\rm CCone$\,$} }
    \newcommand    {\cone}  { \mbox{\rm cone$\,$} }
    \newcommand    {\grad}  { \mbox{\rm grad$\,$} }
    \newcommand    {\even}  { \mbox{\rm even$\,$} }
    \newcommand    {\odd}   { \mbox{\rm odd$\,$} }
    \newcommand    {\sonst} { \mbox{\rm sonst$\,$} }
%
%
%%%%%%%%%%%%%%%%%  Spezielle aufwendigere neue Zeichen   %%%%%%
%
%
    \newcommand    {\C}     { \langle }
    \newcommand    {\Z}     { \rangle }

    \newcommand    {\Doe}   { \mbox{
                                \makebox[.2em][c]{$\circ$}---\makebox[.2em][c]
                                                 {$\bullet$}  }}
    \newcommand    {\doe}   { \mbox{
                                \makebox[.2em][c]{$\bullet$}---\makebox[.2em][c]
                                                 {$\circ$}   }}
%
    \newcommand    {\isotone}  {\unitlength1pt
                                    \begin{picture}(28,15)
                                        \put(8,1){  \vector(2,1){12}  }
                                    \end{picture}   }
%
    \newcommand    {\kreuz}[2] {\mbox{ \raisebox{-1.2ex}
                                  {$\stackrel {\stackrel{#2}
                                     { \displaystyle \times}  }
                                  {\scriptscriptstyle {#1}}$}}}
%
    \newcommand    { \lgo }[2] {\begin{array}[t]{c}
                                   \longrightarrow \\ {\raisebox{2ex}[-2ex]
                                      {$\scriptstyle #1 \to #2 $} }
                                \end{array} }
%
    \newcommand    {\tmid}[1]  {\raisebox{1.95ex}[-1.95ex] {#1} }
%
%%%%%
%%%%%
%%%%% End    LaTeX  File PRE_MATH.tex            11. Dec. 95  %%%%%%%%%%%%%%%%%
